ArabianGPT: Native Arabic GPT-based Large Language Model

The predominance of English and Latin-based large language models (LLMs) has led to a notable deficit in native Arabic LLMs. This discrepancy is accentuated by the prevalent inclusion of English tokens in existing Arabic models, detracting from their efficacy in processing native Arabic's intricate morphology and syntax. Consequently, there is a theoretical and practical imperative for developing LLMs predominantly focused on Arabic linguistic elements. To address this gap, this paper proposes ArabianGPT, a series of transformer-based models within the ArabianLLM suite designed explicitly for Arabic. These models, including ArabianGPT-0.1B and ArabianGPT-0.3B, vary in size and complexity, aligning with the nuanced linguistic characteristics of Arabic. The AraNizer tokenizer, integral to these models, addresses the unique morphological aspects of Arabic script, ensuring more accurate text processing. Empirical results from fine-tuning the models on tasks like sentiment analysis and summarization demonstrate significant improvements. For sentiment analysis, the fine-tuned ArabianGPT-0.1B model achieved a remarkable accuracy of 95%, a substantial increase from the base model's 56%. Similarly, in summarization tasks, fine-tuned models showed enhanced F1 scores, indicating improved precision and recall in generating concise summaries. Comparative analysis of fine-tuned ArabianGPT models against their base versions across various benchmarks reveals nuanced differences in performance, with fine-tuning positively impacting specific tasks like question answering and summarization. These findings underscore the efficacy of fine-tuning in aligning ArabianGPT models more closely with specific NLP tasks, highlighting the potential of tailored transformer architectures in advancing Arabic NLP.

==> 01_old_related_works.tex <==
\section{Related Works}\label{sec2}

The development of Generative Pre-trained Transformers (GPTs) in Natural Language Processing (NLP) has predominantly hinged on the utility of Causal Language Modeling (CLM) as a fundamental pre-training methodology. 
The success of Generative Pre-trained Transformers (GPTs) in Natural Language Processing (NLP) stems from their reliance on CLM as a pre-training technique. 
% GPT-1 \cite{RAD2018} demonstrated CLM's effectiveness in improving generalization capabilities, while GPT-2 \cite{RAD2019} further showcased the power of scaling: with a larger model and dataset, it surpassed state-of-the-art performance on many tasks in a zero-shot setting \cite{BRO2020}. GPT-3 \cite{BRO2020}, with its 175 billion parameters, pushed this approach to the extreme, utilizing CLM and terabytes of internet text. 
It also explored few-shot learning, where a text prompt instructs the model on a new task, unlocking novel capabilities at test time. However, this scaling approach has downsides. The high computational cost and vast corpora required for pre-training limit large models primarily to English.
The inception of GPT-1 \cite{RAD2018} was a pivotal moment, demonstrating the efficacy of CLM in enhancing the generalization capabilities of language models. The subsequent iteration, GPT-2 \cite{RAD2019}, expanded this premise by embracing scalability, wherein an augmented model size coupled with an extensive dataset facilitated a surpassing of existing benchmarks in several NLP tasks without prior specific task training, as detailed in \cite{BRO2020}. GPT-3’s introduction, with its unprecedented 175 billion parameters, further extrapolated this approach, incorporating a voluminous corpus of internet-based text and delving into the realms of few-shot learning, thereby enabling the model to acquire new task capabilities guided by minimal textual prompts.


Despite these advancements, the scaling strategy inherent in these models has its limitations, primarily the substantial computational resources and the extensive corpora required for effective pre-training. This constraint has predominantly restricted the development of such large models to the English language, creating a notable gap in the landscape of multilingual NLP, especially for languages with intricate linguistic features like Arabic.
In the context of Arabic NLP, the concept of transfer learning has gained traction, exemplified by the development of Hulmona, an Arabic Universal Language Model \cite{ELJ2019}. Utilizing a 3-layer AWD-LSTM model structure and training on a corpus of 600K pre-segmented Wikipedia articles using MADAMIRA \cite{PAS2014}.
This approach of fine-tuning on language-specific datasets represents an effort to tailor general models to the nuances of Arabic.



The domain of Arabic natural language processing (NLP) has witnessed significant advancements with the introduction of various LLMs, each contributing uniquely to the field. However, the integration of substantial English tokens in these models often hampers their efficacy in processing the intricate morphology and syntax of native Arabic. Our ArabianGPT model addresses this gap by focusing predominantly on Arabic linguistic elements, offering a nuanced approach to Arabic NLP.
Jais and Jais-chat \cite{SEN2023} represent notable efforts in Arabic-centric LLMs, utilizing a bilingual training approach. Their specialized data processing and technological adaptations for Arabic text are commendable. However, the considerable English data inclusion might dilute their capacity to fully capture the morphological nuances of Arabic, an aspect where ArabianGPT, with its primary focus on Arabic, potentially offers a more comprehensive understanding of Arabic syntax and morphology.

Besides, a few attempts have been made to create an Arabic Transformer-based CLM \cite{ANT2020b} \cite{NAG2022} \cite{SEN2023}. While these approaches demonstrate Arabic text generation capabilities, they may not be optimal for the language due to inherent limitations of pre-training on predominantly English data.

AceGPT \cite{huang2023acegpt}, targeting cultural sensitivity and local values in the Arabic-speaking community, adopts an approach encompassing pre-training with Arabic texts and Supervised Fine-Tuning (SFT). While it significantly addresses cultural alignment, AceGPT might not be as adept in handling the linguistic diversity within the Arabic language. ArabianGPT's design, aligning with the nuanced linguistic characteristics of Arabic, could offer superior performance in language-specific tasks.

AraGPT2 \cite{antoun2020aragpt2}, as a model trained on a large corpus of Arabic internet text and news articles, marks a significant step in Arabic language generation models. Its focus on internet and news texts might, however, limit its understanding of classical and dialectal Arabic. ArabianGPT's diverse training dataset, encompassing both classical and modern standard Arabic, provides a broader linguistic coverage.

AraBERT \cite{ANT2020a}, employing a BERT-based \cite{devlin2018bert} approach, sets new standards in Arabic NLP tasks like sentiment analysis and named entity recognition. Nevertheless, its potential limitations in generative capabilities are areas where ArabianGPT could excel, particularly with its focus on generative tasks such as text generation and summarization.

JASMINE \cite{abdul2023jasmine} offers a suite of models for Arabic, emphasizing societal impacts and biases, alongside a comprehensive benchmark for evaluation. While it addresses social biases effectively, JASMINE may not be tailored specifically to the linguistic needs of Arabic as ArabianGPT, which is designed with a deep focus on Arabic morphological structures.

CAMeLBERT \cite{inoue2021interplay} and AraELECTRA \cite{antoun2020araelectra}, with their exploration of variant effects in pre-trained language models and innovative training objectives, respectively, have pushed the boundaries of Arabic NLP. However, their scope might be limited in generative tasks, a domain where ArabianGPT’s transformer-based approach, specifically designed for generative tasks, could provide enhanced performance.

Models like GigaBERT \cite{lan2020empirical} and ARBERT \& MARBERT \cite{abdul2020arbert}, focusing on bilingual and dialectal aspects of Arabic, have improved understanding and transfer learning capabilities. Yet, their primary emphasis on understanding and extraction tasks may not fully address the generative capabilities, an area where ArabianGPT aims to contribute significantly with its specialized focus.

Lastly, models such as QARiB \cite{abdelali2021pre}, JABER \& SABIR \cite{ghaddar2022revisiting}, and AraT5 \cite{nagoudi2021arat5} have addressed various aspects of Arabic NLP, from dialectal variety to text-to-text transformation capabilities. While making substantial strides in their respective areas, their emphasis might not be as heavily placed on pure Arabic generative tasks as with ArabianGPT.

These models, while demonstrating capabilities in Arabic text generation, often encounter the challenge of pre-training on data that is predominantly English, limiting their effectiveness for Arabic language processing. By contrast, ArabianGPT’s focus on purely Arabic generative tasks, combined with its deep understanding of Arabic morphology and syntax, uniquely positions it to bridge the existing gap in processing and generating native Arabic text. ArabianGPT's specialized AraNizer tokenizer further enhances its capability in handling the unique morphological aspects of Arabic, offering a distinct advantage in terms of accuracy in text processing for tasks like sentiment analysis and summarization.



% Furthermore, the adaptation of Masked Language Modeling (MLM), a variant of CLM where the model predicts a masked word within a sequence, has shown promise in pre-training Arabic Natural Language Understanding (NLU) models. Notable examples include ARABERT \cite{ANT2020a}, Arabic-BERT \cite{SAF2020}, MarBERT \cite{ABD2020}, and QARiB \cite{abdelali2021pre}. 



Consequently, the ArabianGPT model emerges as a significant contribution within the ArabianLLM series. Its design aligns with the architecture of GPT-2 \cite{RAD2019}, but it is distinctively tailored to cater to the Arabic language's unique syntactic and morphological complexities. ArabianGPT sets itself apart by focusing on comprehensive language processing specifically for Arabic, a linguistic domain that has been relatively underserved in the context of advanced LLMs.


The development of ArabianGPT also underscores a commitment to ethical considerations and responsible deployment in NLP. This approach aligns with the increasing focus on ethical practices in AI and language technology, particularly in addressing the needs of diverse linguistic communities. By prioritizing linguistic inclusivity and cultural nuances, ArabianGPT aims to not only bridge technological gaps but also address broader concerns about representation and fairness in NLP.
ArabianGPT's innovation is further exemplified in its integration of specialized tokenization strategies, specifically





% Masked Language Modeling (MLM), a slight variation on CLM where the system predicts a masked word within a sequence, has also proved beneficial for pre-training Arabic NLU models. Examples include ARABERT \cite{ANT2020a}, Arabic-BERT \cite{SAF2020}, MarBERT \cite{ABD2020}, and QARiB \cite{CHO2020}. 


Thus, ArabianGPT's development stands upon the shoulders of several key advancements in the realm of large language models for Arabic. Its core architecture echoes that of GPT-2 \cite{RAD2019}, a moderate-size, yet powerful and versatile pre-trained model originally conceived for English text generation. ArabianGPT, however, forms part of the broader ArabianLLM series, where each model within the series, like ArabianGPT 0.1B and 0.3B, targets different levels of computational and linguistic complexity to cater to a wider spectrum of applications. Furthermore, the development of ArabianGPT prioritizes ethical considerations and responsible deployment, harmonizing with the burgeoning focus on ethical NLP practices across diverse languages and domains.

Beyond its core architecture, ArabianGPT draws inspiration and leverages techniques from a multitude of sources. The model incorporates specialized tokenization and handling of morphological and syntactic features specific to the Arabic language, drawing upon cutting-edge advancements in Arabic NLP research \cite{ANT2020a} \cite{ABD2020}.

By building upon these established foundations and forging its own path through tailored innovations for Arabic, ArabianGPT strives to push the boundaries of natural language understanding and generation for the Arabic language. This marks a significant step forward in unlocking the expressive power and intricate beauty of Arabic, paving the way for a wealth of new applications and advancements in communication, creativity, and knowledge discovery.
